TABBIE: Pretrained Representations of Tabular Data

Existing work on tabular representation learning jointly models tables and associated text using self-supervised objective functions derived from pretrained language models such as BERT. While this joint pretraining improves tasks involving paired tables and text (e.g., answering questions about tables), we show that it underperforms on tasks that operate over tables without any associated text (e.g., populating missing cells). We devise a simple pretraining objective (corrupt cell detection) that learns exclusively from tabular data and reaches the state-of-the-art on a suite of table based prediction tasks. Unlike competing approaches, our model (TABBIE) provides embeddings of all table substructures (cells, rows, and columns), and it also requires far less compute to train. A qualitative analysis of our model's learned cell, column, and row representations shows that it understands complex table semantics and numerical trends.

==> figs/ctp_ana.tex <==
\makeatother
\begin{figure}[t]
    \centering
  \includegraphics[width=1.0\linewidth]{figs/ctp_ana_.pdf}
  \caption{The blue bar graph is the number of tabbie errors and the orange bar graph is the number of tabert errors. There are also no clear differences between the two models for each column.}
  \label{fig:ctp_ana}
\end{figure}


==> figs/name_col.tex <==
\makeatother
\begin{figure}[t]
    \centering
 % \begin{flushleft}
  \includegraphics[width=1.0\linewidth]{figs/name_col_.png}
  \caption{clustering results for the "name" column embedding. We extract the most frequent eight column combinations that include "name" column. (left) clustering results of TaBERT, (right) clustering results of \name\ mix model.}
  \label{fig:name_col}
 % \end{flushleft}
\end{figure}


==> figs/nn_row.tex <==
\makeatother
\begin{figure}[t]
    \centering
 % \begin{flushleft}
  \includegraphics[width=0.75\linewidth]{figs/nn_row_.pdf}
  \caption{nearest neighbor result of row embeddings.}
  \label{fig:nn_row}
 % \end{flushleft}
\end{figure}


==> figs/num_understand2.tex <==
\makeatother
\begin{figure}[t]
    \centering
 %\begin{center}
  \includegraphics[width=1.0\linewidth]{figs/num_understand2_.pdf}
  \caption{corrupted cell probability of the date column.}
  \label{fig:num_understand2}
 % \end{center}
\end{figure}


==> tables/exp_cp_old.tex <==
\todo{H: merge row/col population result tables}

\begin{table}
\centering
\scalebox{0.83}{
\begin{tabular}{lcccccccc}
\hline
N & Method & MAP & MRR & Ndcg-10 & Ndcg-20 \\
\hline
\multirow{4}{*}{ 1 }  & BL & {25.1} & {37.5} & {-}& {-}  \\
& BL+TH & {25.5} & {0.38.0} & {27.1} & {31.5}  \\
& TaBERT & {33.8} & {43.0}  & {36.1} & {39.0} \\ 
& Ours(freq) & {\textbf{36.3}} & {\textbf{48.0}}  & {\textbf{39.5}} & {\textbf{41.9}} \\ 
& Ours(mix) & {35.5} & {46.9}  & {38.5} & {41.3} \\ \hline
\multirow{4}{*}{  2 }  & BL & {28.5} & {40.4} & {-}& {-}  \\
& BL+TH & {33.2} & {44.0} & {36.1} & {41.3}  \\
& TaBERT & {50.8} & {60.0}  & {54.4} & {56.5} \\
& Ours(freq) & {\textbf{51.3}} & {\textbf{61.7}}  & {\textbf{55.1}} & {\textbf{57.0}} \\ 
& Ours(mix) & {51.0} & {61.5}  & {54.8} & {56.6} \\ \hline
\multirow{4}{*}{ 3 }  & BL & {28.5} & {35.5} & {-}& {-}  \\
& BL+TH & {40.0} & {50.8} & {45.2} & {48.5}  \\
& TaBERT & {53.3} & {61.1}  & {57.0} & {58.0} \\
& Ours(freq) & {\textbf{54.1}} & {\textbf{62.5}}  & {\textbf{57.5}} & {\textbf{58.6}} \\ 
& Ours(mix) & {53.6} & {61.6}  & {57.0} & {58.0} \\ \hline

\end{tabular}%
}
%}
\caption{Accuracy of column population}\label{tab:exp_cp}
\end{table}


==> tables/exp_ctp_full.tex <==
\begin{table}
\centering
\begin{tabular}{lccc}
\hline
Method & f1-score \\
\hline
\verb|Sherlock| \cite{Hulsebos2019SherlockAD} & {0.867} \\
\verb|Sato| \cite{zhang2019sato} & {0.908} \\
\verb|TaBERT| \cite{yin20acl} & {0.972} \\
\verb|Ours(freq)| & {0.969} \\ 
\verb|Ours(mix)| & {0.967} \\ \hline

\end{tabular}
\caption{Support weighted f1-score of the column type prediction}\label{tab:exp_ctp_full}
\end{table}

\todo{I noticed the wrong setting for TaBERT n=57600. I modified it and update the result(before: epoch10, after: epoch15)}


==> tables/exp_fcd_header.tex <==
\begin{table}
\centering
\scalebox{0.95}{
\begin{tabular}{lcccccccc}
\hline
method & prediction & recall & f1-score\\
\hline
TaBERT & {94.0} & {85.0} & {89.3}  \\ 
Ours(freq) & {99.4} & {99.6}  & \textbf{{99.5}}  \\ 
Ours(mix) & {99.5} & {99.6}  & \textbf{{99.5}}  \\ \hline
\end{tabular}%
}
%}
\caption{The result of corrupt header detection}\label{tab:exp_fcd_header}
\end{table}


==> tables/exp_pop.tex <==
\todo{H: merge row/col population result tables}

\begin{table*}
\centering
\scalebox{0.85}{
\begin{tabular}{lccccc|cccccccc}
\hline
\multicolumn{6}{c|}{Column population} & \multicolumn{5}{c}{Row population} \\ \hline
N & Method & MAP & MRR & Ndcg-10 & Ndcg-20 & N & Method & MAP & MRR & Ndcg-10 & Ndcg-20 \\
\hline
\multirow{4}{*}{ 1 }  & GPM & {25.1} & {37.5} & {-}& {-} & \multirow{4}{*}{ 1 } \\
& GPM+TH & {25.5} & {0.38.0} & {27.1} & {31.5}  \\
& TaBERT & {33.1} & {41.3}  & {35.1} & {38.1} \\ 
& Ours(freq) & {\textbf{37.9}} & {\textbf{49.1}}  & {\textbf{41.2}} & {\textbf{43.8}} \\ 
& Ours(mix) & {37.1} & {48.7}  & {40.4} & {43.1} \\ \hline
\multirow{4}{*}{  2 }  & GPM & {28.5} & {40.4} & {-}& {-}  \\
& GPM+TH & {33.2} & {44.0} & {36.1} & {41.3}  \\
& TaBERT & {51.1} & {60.1}  & {54.7} & {56.6} \\
& Ours(freq) & {\textbf{52.0}} & {\textbf{62.8}}  & {\textbf{55.8}} & {\textbf{57.6}} \\ 
& Ours(mix) & {51.7} & {62.3}  & {55.6} & {57.2} \\ \hline
\multirow{4}{*}{ 3 }  & GPM & {28.5} & {35.5} & {-}& {-}  \\
& GPM+TH & {40.0} & {50.8} & {45.2} & {48.5}  \\
& TaBERT & {53.3} & {60.9}  & {56.9} & {57.9} \\
& Ours(freq) & {\textbf{54.5}} & {\textbf{63.3}}  & {\textbf{57.9}} & {\textbf{58.9}} \\ 
& Ours(mix) & {54.1} & {62.3}  & {57.4} & {58.7} \\ \hline

\end{tabular}%
}
%}
\caption{result of population taks}\label{tab:exp_pop}
\end{table*}

